A Semi-Implicit Variational Multiscale Formulation for the Incompressible Navier-Stokes Equations via Exact Adjoint Linearization

A semi-implicit, residual-based variational multiscale (VMS) formulation is developed for the incompressible Navier-Stokes equations. The convection term is linearized using an extrapolated (Oseen-type) convecting velocity, producing a linear advection operator whose adjoint can be written exactly. Because of this exact adjoint, unresolved-scale contributions enter the weak form without spatial derivatives of the fine-scale velocity, thereby eliminating the case-by-case adjustments that often accompany nonlinear residual-based VMS implementations. The formulation is presented for a generalized linear convection operator encompassing the convective, skew-symmetric, and divergence forms. Since the discrete method is linear by construction and monolithic for velocity and pressure, each time step requires only one linear solve, reducing wall-clock time by a factor of $2$ to $5$ relative to fully implicit nonlinear formulations while maintaining comparable accuracy. Temporal convergence is verified, and validation is performed on the lid-driven cavity, flow past a cylinder, turbulent channel flow, and flow over a NACA0012 airfoil at a high Reynolds number, demonstrating the efficiency of the proposed approach on problems of practical scale.

==> CF_Plots/cf27_urms_Re395.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=0.95\textwidth,
    height=0.24\textwidth,
    xlabel={$y^+$},
    ylabel={$u_{x,\mathrm{rms}}^+$},
    xmin=0,
    xmax=400,
    ymin=0,
    ymax=4,
    grid=both,
    grid style={dotted},
    line width=1pt,
    mark size=3pt,
    every mark/.append style={solid, line width=0.7pt},
    tick label style={font=\normalsize},
    label style={font=\normalsize},
    legend style={
        font=\small,
        draw=none,
        fill=none
    },
    legend to name=cfRe395FluctuationLegend,
    legend columns=3,
    legend cell align=left,
]

% --- linear S = 0
\addplot[black, solid, mark=triangle, mark repeat=3, mark phase=2]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r11}), col sep=comma, header=true]
{CF_InputData/C203_Linear_Re395_S0_RR.csv};
\addlegendentry{linear, $s=0$}

% --- linear S = 0.5
\addplot[ForestGreen, solid, mark=diamond, mark repeat=3, mark phase=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r11}), col sep=comma, header=true]
{CF_InputData/C204_Linear_Re395_S0P5_RR.csv};
\addlegendentry{linear, $s=0.5$}

% --- linear S = 1
\addplot[Purple, solid, mark=pentagon, mark repeat=3, mark phase=4]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r11}), col sep=comma, header=true]
{CF_InputData/C205_Linear_Re395_S1_RR.csv};
\addlegendentry{linear, $s=1$}

% --- nonlinear S = 0 (stored as mean-square fluctuation)
\addplot[blue, solid, mark=o, mark repeat=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r11}), col sep=comma, header=true]
{CF_InputData/C201_nonLinear_Re395_S0_RR.csv};
\addlegendentry{nonlinear, $s=0$}

% --- nonlinear S = 1
\addplot[red, solid, mark=square, mark repeat=3, mark phase=1]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r11}), col sep=comma, header=true]
{CF_InputData/C202_nonLinear_Re395_S1_RR.csv};
\addlegendentry{nonlinear, $s=1$}

% Keep the nonlinear entries together on the second legend row.
\addlegendimage{empty legend}
\addlegendentry{}

% --- Bazilevs et al. VMS/NURBS, $64^3$
\addplot[
    BurntOrange,
    very thick,
    dashdotted,
    mark=star,
    mark size=4pt,
    mark repeat=4,
    mark phase=3
]
table[
    x=y+,
    y=u_rms_plus,
    col sep=comma,
    header=true
]{CF_InputData/Bazilevs_Linear_Re395_64_Fluctuations.csv};
\addlegendentry{Bazilevs et al. (VMS)}

% --- Moser DNS (stored as mean-square fluctuation)
\addplot[black, very thick, mark=none]
table[
    x=y+,
    y expr=sqrt(\thisrow{R_uu}),
    col sep=comma,
    header=true
]{CF_InputData/chan395.reystress.csv};
\addlegendentry{Moser et al. (1999) DNS}

\end{axis}
\end{tikzpicture}


==> CF_Plots/cf28_vrms_Re395.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=0.95\textwidth,
    height=0.24\textwidth,
    xlabel={$y^+$},
    ylabel={$u_{y,\mathrm{rms}}^+$},
    xmin=0,
    xmax=400,
    ymin=0,
    ymax=1.2,
    grid=both,
    grid style={dotted},
    line width=1pt,
    mark size=3pt,
    every mark/.append style={solid, line width=0.7pt},
    tick label style={font=\normalsize},
    label style={font=\normalsize},
]

% --- linear S = 0
\addplot[black, solid, mark=triangle, mark repeat=3, mark phase=2]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r22}), col sep=comma, header=true]
{CF_InputData/C203_Linear_Re395_S0_RR.csv};

% --- linear S = 0.5
\addplot[ForestGreen, solid, mark=diamond, mark repeat=3, mark phase=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r22}), col sep=comma, header=true]
{CF_InputData/C204_Linear_Re395_S0P5_RR.csv};

% --- linear S = 1
\addplot[Purple, solid, mark=pentagon, mark repeat=3, mark phase=4]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r22}), col sep=comma, header=true]
{CF_InputData/C205_Linear_Re395_S1_RR.csv};

% --- nonlinear S = 0
\addplot[blue, solid, mark=o, mark repeat=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r22}), col sep=comma, header=true]
{CF_InputData/C201_nonLinear_Re395_S0_RR.csv};

% --- nonlinear S = 1
\addplot[red, solid, mark=square, mark repeat=3, mark phase=1]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r22}), col sep=comma, header=true]
{CF_InputData/C202_nonLinear_Re395_S1_RR.csv};

% --- Bazilevs et al. VMS/NURBS, $64^3$
\addplot[
    BurntOrange,
    very thick,
    dashdotted,
    mark=star,
    mark size=4pt,
    mark repeat=4,
    mark phase=3
]
table[x=y+, y=v_rms_plus, col sep=comma, header=true]
{CF_InputData/Bazilevs_Linear_Re395_64_Fluctuations.csv};

% --- Moser DNS (stored as mean-square fluctuation)
\addplot[black, very thick, mark=none]
table[x=y+, y expr=sqrt(\thisrow{R_vv}), col sep=comma, header=true]
{CF_InputData/chan395.reystress.csv};

\end{axis}
\end{tikzpicture}


==> CF_Plots/cf29_wrms_Re395.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=0.95\textwidth,
    height=0.24\textwidth,
    xlabel={$y^+$},
    ylabel={$u_{z,\mathrm{rms}}^+$},
    xmin=0,
    xmax=400,
    ymin=0,
    ymax=1.5,
    grid=both,
    grid style={dotted},
    line width=1pt,
    mark size=3pt,
    every mark/.append style={solid, line width=0.7pt},
    tick label style={font=\normalsize},
    label style={font=\normalsize},
]

% --- linear S = 0
\addplot[black, solid, mark=triangle, mark repeat=3, mark phase=2]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r33}), col sep=comma, header=true]
{CF_InputData/C203_Linear_Re395_S0_RR.csv};

% --- linear S = 0.5
\addplot[ForestGreen, solid, mark=diamond, mark repeat=3, mark phase=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r33}), col sep=comma, header=true]
{CF_InputData/C204_Linear_Re395_S0P5_RR.csv};

% --- linear S = 1
\addplot[Purple, solid, mark=pentagon, mark repeat=3, mark phase=4]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r33}), col sep=comma, header=true]
{CF_InputData/C205_Linear_Re395_S1_RR.csv};

% --- nonlinear S = 0
\addplot[blue, solid, mark=o, mark repeat=3]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r33}), col sep=comma, header=true]
{CF_InputData/C201_nonLinear_Re395_S0_RR.csv};

% --- nonlinear S = 1
\addplot[red, solid, mark=square, mark repeat=3, mark phase=1]
table[x expr=\thisrow{y}*395, y expr=sqrt(\thisrow{r33}), col sep=comma, header=true]
{CF_InputData/C202_nonLinear_Re395_S1_RR.csv};

% --- Bazilevs et al. VMS/NURBS, $64^3$
\addplot[
    BurntOrange,
    very thick,
    dashdotted,
    mark=star,
    mark size=4pt,
    mark repeat=4,
    mark phase=3
]
table[x=y+, y=w_rms_plus, col sep=comma, header=true]
{CF_InputData/Bazilevs_Linear_Re395_64_Fluctuations.csv};

% --- Moser DNS (stored as mean-square fluctuation)
\addplot[black, very thick, mark=none]
table[x=y+, y expr=sqrt(\thisrow{R_ww}), col sep=comma, header=true]
{CF_InputData/chan395.reystress.csv};

\end{axis}
\end{tikzpicture}

